On the complexity of finding set repairs for data-graphs

In the deeply interconnected world we live in, pieces of information link domains all around us. As graph databases embrace effectively relationships among data and allow processing and querying these connections efficiently, they are rapidly becoming a popular platform for storage that supports a wide range of domains and applications. As in the relational case, it is expected that data preserves a set of integrity constraints that define the semantic structure of the world it represents. When a database does not satisfy its integrity constraints, a possible approach is to search for a 'similar' database that does satisfy the constraints, also known as a repair. In this work, we study the problem of computing subset and superset repairs for graph databases with data values using a notion of consistency based on a set of Reg-GXPath expressions as integrity constraints. We show that for positive fragments of Reg-GXPath these problems admit a polynomial-time algorithm, while the full expressive power of the language renders them intractable.

==> drawings/dataRepresentationExample.tex <==
\label{representation:dataTree}
\begin{figure} [H]
\centering
    \begin{tikzpicture}[node distance={20mm}, thick, main/.style = {draw, circle}] 
\node[main] (1) {1}; 
\node[main] (2) [below left of=1] {11}; 
\node[main] (3) [below right of=1] {12}; 
\node[main] (4) [below of=3] {121};
\node[draw] at (0,0) {some text};
\node[draw] at (-2,0) {some text\\ lines};
\draw[->] (1) -- (2);
\draw[->] (1) -- (3);
\draw[->] (3) -- (4);

%\draw[->] (6) -- node[midway, above right, sloped, pos=1] {+1} (4); 
\end{tikzpicture} 
\caption{Caption}
\end{figure}

==> expTimeProof.tex <==
\begin{theorem}\label{teo:ExpTime}

    The problem $\exists$\textsc{SUPERSET-REPAIR} is \textsc{ExpTime}-hard when $\mathcal{L} = \Gregxpath$

\end{theorem}

\begin{proof} In order to prove this theorem, we use another result obtained in \cite{figueira2012decidability} related to the satisfiability problem for \textbf{Downward XPath}. Basically this problem consists in deciding, given a downward-XPath formula, if there exists a data tree such that the expression is satisfied at the root. A data tree in that context is defined as a tuple $<\mathcal{T},\sigma,\delta>$ where $\mathcal{T}$ is a non-empty, prefix-closed set of elements from $\N^*$ representing the nodes from the tree such that whenever $x(i+1) \in \mathcal{T}$ then $xi \in \mathcal{T}$; $\sigma: \mathcal{T} \to \Sigma$ is a labeling function and $\delta: \mathcal{T} \to \triangle$ is a data value function. $\Sigma$ must be a finite set, and $\triangle$ a countable one.

We consider the fact that the satisfiability problem for XPath$(\down^*, =)$ node formulas, given by the grammar:

\begin{center}
    $\aPath, \aPathb$ = $o$ $|$ $\aPath [\aFormula]$ $|$ $[\aFormula] \aPath$ $|$  $\aPath$ . $\aPathb$ $|$ $\aPath \pathUnion \aPathb$  \hspace{0.5cm} $o \in \{\down^*, \epsilon\}$
\end{center}

\begin{center}
    $\aFormula, \aFormulab$ = $a$ $|$ $\neg \aFormula$ $|$ $\aFormula \wedge \aFormulab$ $|$ $\comparacionCaminos{\aPath}$ $|$ $\comparacionCaminos{\aPath = \aPathb}$ $|$ $\comparacionCaminos{\aPath \neq \aPathb}$ \hspace{0.5cm} $a \in \Sigma_s$
\end{center}

is \textsc{ExpTime-complete}. We observe that the data trees considered in \cite{figueira2012decidability} have both labels and data values associated to each node. This is important when considering the semantics of XPath$(\down^*,=)$ expressions, since the node expression $a$ is true for every node having label equal to $a$ (that is, $\sigma(v)=a$) while the path comparison expression $\comparacionCaminos{\aPath = \aPathb}$ is true for those nodes $v$ that can reach tho nodes $w$ and $z$ respectively via $\aPath$ and $\aPathb$ such that their data values are equal (that is, $\delta(w) = \delta(z)$). The $\neq$ semantics are analogous.

We will reduce the satisfiability problem for XPath($\down^*, =$) to \textsc{$\exists$SUPERSET-REPAIR} for $\mathcal{L} = \Gregxpath$. To do this, given a XPath($\down^*, =$) node expression $\aFormula$, we will define a data-graph $\aGraph$, a set $\aRestrictionSet$ of \Gregxpath expressions and a $\Gregxpath$ node expression $\aFormula'$ such that every superset repair of $\aGraph$ with respect to $\aRestrictionSet$ will represent a data tree, and if this data tree satisfies $\aFormula'$ then we will be able to reconstruct a tree for the satisfiability problem.

First, we will define our fixed sets $\Sigma_e$ and $\Sigma_n$. They will be related to the fixed sets of \textit{symbols} and \textit{data values} from the \textbf{downward XPath} problem: $\Sigma_s$ and $\triangle$ respectively ($\Sigma_s$ is finite, while $\triangle$ is not). In the tree setup, there is only one kind of edge, which we will call \esLabel{down} edge. We will also use two extra types of edges: \esLabel{root} and \esLabel{value} edges. The first will be used to distinguish a special root from the data-graph $\aGraph$, while the second one to simulate the data values from the trees. Therefore, we define $\Sigma_e = \{\esLabel{down}, \esLabel{value}, \esLabel{root}\}$. 

Meanwhile, we will define $\Sigma_n = \Sigma_s \cup \triangle \cup \{r\}$, where $r$ is a distinguished value for the root of $\aGraph$. That is, both symbols and data values will be simulated via the data values from the nodes. To do this, we will force a specific structure to repairs using the \Gregxpath constraints.

Our initial data-graph $\aGraph$ is defined in the following way: $\aGraph = (V,L,D)$ where $V = \{$ $v_c$ $|$ $c \in \Sigma_s \cup \{r\}$\}, $L(v_r, v_c) = \{\esLabel{root}\}$ for $c \in \Sigma_s$ and $L(v,w) = \emptyset$ for every other pair of nodes, and $D(v_c) = c$ for $c \in \Sigma_s \cup \{r\}$. Note that this data-graph does not have any cycles, and can be considered an arborescence where $v_r$ is the root.

The idea is that in a valid superset repair there must be a child $z$ from $v_r$ connected through a $\esLabel{root}$ edge such that the subtree rooted at $z$ is a representation of a tree that satisfies the input downward XPath formula $\aFormula$. Hence, we need to add restrictions to make sure that every repair will satisfy this condition.  

To ensure that every superset repair keeps being an arborescence rooted at $r$ and that it does not use the \esLabel{root} edges we will use the following restrictions:

\begin{itemize} 

    \item $\aPath_{connected} = (\_^*\_^{-*})^*$: the graph should be connected.
    
    \item $\aPath_{noCycles} = \epsilon \entoncesCamino \overline{\_^+}$: the graph should not have directed cycles.
    
    \item $\aPath_{0or1parents} = \_ $. 
    $ \_^- \entoncesCamino \epsilon$: every node should have a unique ancestor.
    
    \item $\aFormulab_{root} = [r^=] \entoncesNodo \lnot \comparacionCaminos{\_^-}$: the node $v_r$ will not have any incoming edges, and therefore will be the root.
    
    \item $\aFormulab_{rootEdges} = \comparacionCaminos{\down_{\esLabel{root}}} \entoncesNodo [r^=]$: any \esLabel{root} edge must begin at $v_r$.
    
\end{itemize}

In some expressions we used $\labelComodin^-$ which is not actually included in the \Gregxpath grammar. To simulate it, we could enumerate every edge label, since we  defined $\Sigma_e$ as a finite set.



We need to adapt our data-graphs so that they can simulate having data values and labels at nodes. Each node from the data-graph will have an outgoing \esLabel{value} edge directed to a node that contains its data value. We need to ensure four things: the nodes from the tree should only use data values from $\Sigma_s$, no `value' node can have any children, every `value' node has to have a data value from $\triangle$ and every tree node must have a unique edge to a `value' node. We can force all this conditions with the following contraints:

\begin{itemize}
    \item $\aFormulab_1 = \down_\esLabel{down}^{-*}\down_{\esLabel{root}}^-[r^=] \entoncesCamino \bigvee\limits_{c \in \Sigma_s} [c^=]$.
    
    \item $\aFormulab_2 = \bigwedge\limits_{c \in \Sigma_s \cup \{r\}} [c^{\neq}] \entoncesNodo \lnot \comparacionCaminos{\down_\esLabel{down}} \wedge \lnot \comparacionCaminos{\down_\esLabel{value}}$
    
    \item $\aFormulab_3 = \comparacionCaminos{\down_\esLabel{value}^-} \entoncesNodo \bigwedge\limits_{c \in \Sigma_s \cup \{r\}} [c^{\neq}]$
    
    \item $\aFormulab_4^1 = \bigvee\limits_{c \in \Sigma_s} [c^=] \entoncesNodo \comparacionCaminos{\down_\esLabel{value}}$
    
    \item $\aFormulab_4^2 = \down_\esLabel{value}^- \down_\esLabel{value} \entoncesCamino \epsilon$
    
\end{itemize}

Now we need to adapt the input downward XPath formula $\phi$ to our setup. Let us define a mapping $f$ from downward XPath formulas to $\Gregxpath$ formulas such that:

\begin{itemize}[label=$\circ$]

    \setlength\itemsep{0em}

    \item $f(\epsilon) = \epsilon$
    
    \item $f(\down^*) = \down_\esLabel{down}^*$
    
    \item $f(a) = [a^=]$ for $a \in \Sigma_s$
    
    \item $f(\aPath [\aFormula]) = f(\aPath)[f(\aFormula)]$
    
    \item $f([\aFormula]\aPath) = [f(\aFormula)]f(\aPath)$
    
    \item $f(\aPath . \aPathb) = f(\aPath) . f(\aPathb)$
    
    \item $f(\aPath \cup \aPathb) = f(\aPath) \cup f(\aPathb)$
    
    \item $f(\lnot \aFormula) = \lnot f(\aFormula)$
    
    \item $f(\aFormula \wedge \aFormulab) = f(\aFormula) \wedge f(\aFormulab)$
    
    \item $f(\comparacionCaminos{\alpha}) = \comparacionCaminos{f(\alpha)}$
    
    \item $f(\comparacionCaminos{\aPath = \aPathb}) = \comparacionCaminos{f(\aPath)\down_\esLabel{value} = f(\aPathb)\down_\esLabel{value}}$
    
    \item $f(\comparacionCaminos{\aPath \neq \aPathb}) = \comparacionCaminos{f(\aPath)\down_\esLabel{value} \neq f(\aPathb)\down_\esLabel{value}}$
    
\end{itemize}

$f$ only concatenates a \esLabel{value} edge at the end of the path comparison expressions in order to access the appropiate data value, and replaces the $\down^*$ edges by $\down_{\esLabel{down}}^*$ ones.

The following lemma proves that $f$ is a function which preserves the truth values of $\Gregxpath$ formulas.

\begin{lemma} \label{lemma:treeConversion}
Let $T$ be a labeled data tree (in the sense of \cite{figueira2012decidability}), $T'$ it's representation as a data-graph, and $\eta$ a \textbf{downward XPath} formula. Then $\eta$ is satisfied at the root of $T$ iff $f(\eta)$ is satisfied at the root of $T'$.
\end{lemma}
\begin{proof}
See the Appendix~\S\ref{Appendix}.
\end{proof}

Finally, we define $\aFormula'$, the $\Gregxpath$ expression that forces every superset repair of $\aGraph$ to contain a representation of a tree satisfying $\aFormula$:

\begin{center}
    $\aFormulab_{sat} = [r^=] \entoncesNodo \down_\esLabel{root} f(\aFormula)$
\end{center}

In summary, given a downward XPath formula $\aFormula$ we construct $\aGraph$ and $\aRestrictionSet = \aRestrictionSet_{arbor} \cup \aRestrictionSet_{dataTree} \cup \{\aFormulab_{sat}\}$ where

\begin{center}
    $\aRestrictionSet_{arbor} = \{\aPath_{connected}, \aPath_{noCycles}, \aPath_{0or1parents}, \aFormulab_{root}, \aFormula_{rootEdges}\}$
    
    
    $\aRestrictionSet_{dataTree} = \{\aFormulab_1, \aFormulab_2, \aFormulab_3, \aFormulab_4^1, \aFormulab_4^2\}$.
    
\end{center}

The size of $\aGraph$ depends on $|\Sigma_s|$, which is fixed and finite. The size of $\aRestrictionSet$ depends linearly on both $|\Sigma_s|$ and $|\aFormula|$. 

We are only left to prove that there exists a tree $T$ with root $r_T$ such that $r_T \in \semantics{\aFormula}_T$ iff there exists a superset repair of $\aGraph$ with respect to $\aRestrictionSet$.

$\implies)$ Let $T$ be a tree with root $r_T$ whose symbol is $a \in \Sigma_s$ such that $r_T \in \semantics{\aFormula}_T$. Let $T'$ be it's data-graph conversion with root $r_{T'}$. Then we know that $r_{T'} \in \semantics{f(\aFormula)}_{T'}$. Let's concatenate $T'$ to $\aGraph$ by merging the child of $v_r$ from $\aGraph$ with symbol $a$ with $r_{T'}$. We also add to every other child of $v_r$ an outgoing $\esLabel{value}$ edge to a new node (one new node for each one of $v_r$'s childs) with a data value from $\triangle$. $R$ is satisfied by this data-graph, which means that there exists a superset repair of $\aGraph$ with respect to $\aRestrictionSet$.

$\impliedby)$ Let $\aGraph'$ be a superset repair of $\aGraph$ with respect to $\aRestrictionSet$. Since $\aGraph' \models \aRestrictionSet_{arbor}$ we know that it is an arborescence rooted at $v_r$. Since $\aGraph' \models \aFormulab_{sat}$ there is a child $v_c$ from $v_r$ such that $v_c \in \semantics{f(\aFormula)}_{\aGraph'}$. Since $f(\aFormula)$ only goes `down' we know that $v_c \in \semantics{f(\aFormula)}_{T}$, where $T$ is the arborescence from $\aGraph'$ rooted at $v_c$. Since $\aGraph' \models \aRestrictionSet_{dataTree}$ we know that $T$ has to be a representation of some tree $T'$ that satisfies $\aFormula$ at the root.

\end{proof}

%item $\varphi_{ancestor\_root} = \comparacionCaminos{\labelComodin^{-*} \expNodoEnCamino{\lnot \comparacionCaminos{\labelComodin^{-1}}}}$. All nodes have an ancestor without a father, that is, a `root', 
%\item $\alpha_{single\_root} = \expNodoEnCamino{\lnot \comparacionCaminos{\labelComodin^{-1}}} \entoncesCamino  (\labelComodin^{*}\labelComodin^{-*})^* \expNodoEnCamino{\lnot \comparacionCaminos{\labelComodin^{-1}}} $. This restriction in addition to $\alpha_{connected}$ and $\varphi_{ancestor\_root}$ means that there is a single root. 




==> preferredRepairs.tex <==
In this Section, we propose two different preference criteria to choose over the set of repairs. The first one is based on the assignment of weights, and the second one on lifting an order over the edge labels and data labels to an order between multisets.

\bigsergio{Quizás pasar toda esta sección a un nuevo paper}
\bigsergio{Hay que dar muchas más justificaciones para nuestras decisiones acá}

\subsection{Weight-based preferences} %Citar que ya está en la bibliografía Querying Inconsistent Description Logic Knowledge Basesunder Preferred Repair Semantics

In the manner done in \cite{bienvenu2014querying} for Description Logic knowledge bases, we provide a notion of {\it weight} over graph databases, which can be translated into preferences via the induced ordering.

%\subsubsection{Initial definitions}

%\paragraph{Weights over edges} \sergio{Sacar esto, dejar solo sobre edges y data}
%We consider a weight function $\weight: \Sigma_e \to \N$. %\sergio{Permitir ir a valores negativos es como en Querying Inconsistent Description Logic Knowledge Basesunder Preferred Repair Semantics, pero tambien puede tener sentido tomar solo positivos}.
%\santi{Consultita: Podría ser $\N$? Porque en ese caso se puede hacer una búsqueda binaria del óptimo suponiendo que solucionaste el problema de decisión de `decidir si existe un repair con peso menor a k'. Aparte en el paper Querying Inconsistent Description... también van con $\N$ (página 3 inmediatamente antes de la sección 4)}% Si se permite todo \Q en vez de \Q_{\ge 0}, se promueve agregar todo lo posible de algunos ejes. 
%\sergio{Tenés razón Cité mal, en que usan sobre Q es Preferred explanations for ontology-Mediated queries under existential rules \cite{ceylan2021preferred}}
%We extend the function to a data graph $G = (V,L_e,D)$ by defining: $$\weight(G) = \sum_{x,y \in V} (\sum_{z \in L_e(x,y)} \weight(z))$$ %visto como conjunto
%We say that $G_1 \lessPreferedInducedWeight G_2$ iff $\weight(G_1) < \weight(G_2)$, in which case we say that $G_1$ is \defstyle{\weight-preferred} to $G_2$.


\paragraph{Weights over edges and data} 
%When considering weights that allow for subset and superset repairs, we must take into account for our weight function the possibility that nodes are removed or added, respectively.

When considering a way to select among various possible subset or superset repairs, one approach is to consider that different edge labels and data values are prioritized differently, being assigned different weights that are aggregated to obtain a measure of the weight of a whole data-graph. This aggregated value can then be compared between possible repairs in order to obtain a preferred repair based on the natural ordering of integers.

%This can be done by extending the domain of the weight function so that it takes into account the data available in the nodes: $$\weight: \Sigma_e \sqcup \Sigma_n \to \N$$
We first consider a weight function over edge labels and data values: $$\weight: \Sigma_e \sqcup \Sigma_n \to \N$$

(where $\sqcup$ denotes that the union is disjoint). 

We can then extend this function to any data-graph $G = (V,L_e,D)$ over $\Sigma_e$ and $\Sigma_n$, by defining:
$$\weight(G) = \sum_{x,y \in V} \left(\sum_{z \in L_e(x,y)} \weight(z) \right) + \sum_{x \in V} \weight(D(x))$$

Finally, we define that $G_1 \lessPreferedInducedWeight G_2$ iff $\weight(G_1) < \weight(G_2)$, in which case we say that $G_1$ is \defstyle{\weight-preferred} to $G_2$.

\begin{remark}
Note that having a weight that is uniform on all the data values implies that the weighting function only cares about the cardinality of the nodes. 

Also, having a very high weight for nodes means that, for superset repairs, edges will be added over new nodes, while in subset repairs nodes will be  preferentially removed instead.
\end{remark}

\begin{example}\label{example:WeightsAndRepairs}
Consider a context where data-graphs represent physical networks, and where edges represent connections that can be of two different quality levels (e.g. varying robustness, resistance to physical attacks) which we call $\downarrow_\esLabel{low}$ and $\downarrow_\esLabel{high}$. 
Let $\aRestrictionSet = \{\aPath_{connected\_dir}, \aPath_{2l\rightarrow good}\}$ be a set of restrictions, where $\aPath_{connected\_dir} = \labelComodin^*$ expresses the notion of directed connectedness, and 
$\aPath_{2l\rightarrow good} = \downarrow_\esLabel{low} \downarrow_\esLabel{low}
\pathIntersection
\entoncesCamino \downarrow_\esLabel{high} \downarrow_\esLabel{low} \pathUnion \downarrow_\esLabel{low} \downarrow_\esLabel{high} \pathUnion \downarrow_\esLabel{high} \downarrow_\esLabel{high} \pathUnion \downarrow_\esLabel{high} \pathUnion \downarrow_\esLabel{low}$
%$\aPath_{2l\rightarrow h} = \downarrow_\esLabel{low} \downarrow_\esLabel{low} \entoncesCamino \downarrow_\esLabel{low} \downarrow_\esLabel{low} \expNodoEnCamino{\comparacionCaminos{\downarrow_\esLabel{high}}}$ 
%$\aPath_{3l\rightarrow **h} = \esLabel{low}^{3,3} \entoncesCamino \esLabel{low}\esLabel{low}\esLabel{high} \pathUnion \esLabel{low}\esLabel{high}\esLabel{low} \pathUnion \esLabel{high}\esLabel{low}\esLabel{low} \pathUnion \esLabel{low}\esLabel{high}\esLabel{high} \pathUnion \esLabel{high}\esLabel{high}\esLabel{low} \pathUnion \esLabel{high}\esLabel{low}\esLabel{high} \pathUnion \esLabel{high}^{3,3} $ establishes that after transversing two low-quality edges, it must always be possible to then transverse a high-quality one. 
establishes that if a node can be reached by two low-quality edges, it is also possible to reach it by a `good' path, which we take to mean that it can be reached in only one step or in two steps but using at least one high-quality edge. 


We could consider a weight function that attempts to represent the costs of building nodes and connections in this network. For example, it could assign a uniform weight to all data values $\weight(\aNode) = 20$, a low cost for low-quality connections $\weight(\downarrow_\esLabel{low}) = 1$, and a higher cost for high-quality connections $\weight(\downarrow_\esLabel{high}) = 5$.

Now, given a data-graph $\aGraph$ that does not satisfy the restrictions, a $\weight$-preferred superset repair can be interpreted as the most cost-effective way of making a superset of the network that satisfies the restrictions while minimizing the costs given by $\weight$. For a full example, see Figures~\ref{figure:weightsExampleSetup}, \ref{figure:weightExampleRepair}, and \ref{figure:weightExamplePreferredRepair}.


% \begin{figure} [H]
% \centering
%     \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
% \node[main] (1) {c}; 
% \node[main] (2) [below right of=1] {d}; 
% \node[main] (3) [below left of=1] {b}; 
% \node[main] (4) [right of=1] {e};
% \node[main] (5) [left of=1] {a};
% \draw[->] (3) -- (5) node[midway, above=0.5pt, sloped]{low}; 
% %\draw (1) to [out=135,in=90,looseness=1.5] (5); 
% \draw[->] (4) -- (1) node[midway, above=0.5pt, sloped, pos=0.5]{high}; 
% \draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
% \draw[->] (2) -- (4) node[midway, above=0.5pt, sloped, pos=0.5]{low}; 
% %\draw[->] (6) -- node[midway, above right, sloped, pos=1] {+1} (4); 
% \end{tikzpicture} 
% \caption{An example of a data-graph that satisfies $\aPath_{2l \rightarrow h}$ but doesn't satisfy $\aPath_{connected\_dir}$.}
% \label{figure:weightsExampleSetup}
% \end{figure}

% \begin{figure} [H]
% \centering
%     \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
% \node[main] (1) {c}; 
% \node[main] (2) [below right of=1] {d}; 
% \node[main] (3) [below left of=1] {b}; 
% \node[main] (4) [right of=1] {e};
% \node[main] (5) [left of=1] {a};
% \draw[->] (3) -- (5) node[midway, above=0.5pt, sloped]{low}; 
% %\draw (1) to [out=135,in=90,looseness=1.5] (5); 
% \draw[->] (4) -- (1) node[midway, above=0.5pt, sloped, pos=0.5]{high}; 
% \draw[->] (1) -- (3) node[midway, above=0.5pt, sloped, pos=0.5]{low}; 
% \draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
% \draw[->] (1) -- (5) node[midway, above=0.5pt, sloped, pos=0.5]{low};
% \draw[->, bend left=30] (5) edge node[midway, above=0.5pt, sloped, pos=0.5]{low} (4) ;
% \draw[->] (2) -- (4) node[midway, above=0.5pt, sloped, pos=0.5]{low}; 
% \draw[->, bend left=10] (3) edge node [above=0.3pt, sloped, near start]{low} (4); 
% \end{tikzpicture} 
% \caption{A possible $\weight$ preferred superset repair with respect to the example of Figure \ref{figure:weightsExampleSetup}.} %Adding either the edge $(a,\esLabel{low},e)$ or $(b,\esLabel{low},d)$ would have also worked.}
% \label{figure:weightExampleRepair}
% \end{figure}

\begin{figure} [H]
\centering
    \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
\node[main] (1) {c}; 
\node[main] (2) [below right of=1] {d}; 
\node[main] (3) [left of=1] {b}; 
\node[main] (4) [right of=1] {e};
\draw[->] (3) -- (1) node[midway, above=0.5pt, sloped]{low}; 
%\draw (1) to [out=135,in=90,looseness=1.5] (5); 
\draw[->] (4) edge node[midway, below=0.5pt, sloped, pos=0.5]{high} (1);
%\draw[->, bend left = 30] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{high} (4); 
\draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\draw[->] (3) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{high};
\draw[->] (2) -- (4) node[midway, above=0.5pt, sloped, pos=0.5]{low}; 
%\draw[->] (6) -- node[midway, above right, sloped, pos=1] {+1} (4); 
\end{tikzpicture} 
\caption{A data-graph that does not satisfy $\aPath_{connected\_dir}$ nor $\aPath_{2l\rightarrow good}$ from Example~\ref{example:WeightsAndRepairs}: it is not connected as a directed graph, and the pair $(c,e)$ of nodes is connected via two $\downarrow_\esLabel{low}$ but cannot be connected via a `good' path.}
\label{figure:weightsExampleSetup}
\end{figure}

\begin{figure} [H]
\centering
    \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
\node[main] (1) {c}; 
\node[main] (2) [below right of=1] {d}; 
\node[main] (3) [left of=1] {b}; 
\node[main] (4) [right of=1] {e};
\draw[->] (3) -- (1) node[midway, above=0.5pt, sloped]{low};
\draw[->, loop left] (3) edge node[midway, above=0.5pt, sloped]{low} (3); 
\draw[->] (4) edge node[midway, below=0.5pt, sloped, pos=0.5]{high} (1);
\draw[->, bend left = 30] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{high} (4); 
\draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\draw[->] (3) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{high};
\draw[->] (2) -- (4) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\draw[->, bend right = 50] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{low} (3); 
\end{tikzpicture} 
\caption{A possible $\weight$ superset repair with respect to the example of Figure \ref{figure:weightsExampleSetup}; note that the removal of any of the new edges ends up violating $\aRestrictionSet$. The associated weight of this repair whould be the original weight plus 1 + 1 + 5 (from the added \esLabel{low} and \esLabel{high} edges).}
\label{figure:weightExampleRepair}
\end{figure}


\begin{figure} [H]
\centering
       \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
\node[main] (1) {c}; 
\node[main] (2) [below right of=1] {d}; 
\node[main] (3) [left of=1] {b}; 
\node[main] (4) [right of=1] {e};
\draw[->] (3) -- (1) node[midway, below=0.5pt, sloped]{low};
\draw[->, loop left = 50] (3) edge node[midway, above=0.5pt, sloped]{low} (3); 
%\draw[->, bend left = 50] (3) edge node[midway, above=0.5pt, sloped]{low} (4); 
\draw[->] (4) edge node[midway, below=0.5pt, sloped, pos=0.5]{high} (1);
\draw[->, bend left = 30] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{low} (4); 
\draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\draw[->] (3) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{high};
\draw[->] (2) -- (4) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\draw[->, bend right = 50] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{low} (3); 
\end{tikzpicture} 
\caption{A $\weight$-preferred superset repair with respect to the example of Figure \ref{figure:weightsExampleSetup}. The associated extra weight of this repair whould be 3, and it can be proved that there is no other superset repair with a lower weight.}
\label{figure:weightExamplePreferredRepair}
\end{figure}
\end{example}

\paragraph{Computing \weight-preferred repairs}

We define the following problem:

\begin{center}

\fbox{\begin{minipage}{30em}
  \textsc{Problem}: \textbf{\weight-preferred} $\star$-repair computing

\textsc{Input}: A data-graph $\aGraph$ and a set $\aRestrictionSet$ of $\mathcal{L}$ expressions.

\textsc{Output}: A $\star$-repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ and \textbf{\weight-preferred} over all other repairs.
\end{minipage}}

\end{center}

where $\star \in \{\subseteq, \supseteq\}$. The weight function $\weight$ is fixed, and it should be an `easy' function to compute. That is, we consider that, given a reasonable codification of $x$, $\weight(x) \leq 2^{p(|x|)}$ for every $x$ and some polynomial $p()$, and that the result of $\weight(x)$ can be computed in polynomial time. Other type of restrictions could be made upon $\weight$ (for example, that $\weight(x) \leq q(|x|)$ for some polynomial $q$) depending on the kind of weight function one wants to model, but we note that, without any restriction, $w$ could even be an uncomputable function. 

Now we study both subset and superset repairs independently.

\subsubsection{\weight-preferred subset repairs}

In the context of subset repairs, it is more reasonable to \textbf{maximize} the weight of the repairs rather than minimizing it. The intuition is that we want to preserve as much value as we can from the original data-graph $\aGraph$. 

We define the related decision problem for subset repairs:

\begin{center}

\fbox{\begin{minipage}{30em}
  \textsc{Problem}: \textbf{$K$ \weight-preferred} $\subseteq$-repair computing

\textsc{Input}: A data-graph $\aGraph$, a value $K$ and a set $\aRestrictionSet$ of $\mathcal{L}$ expressions.

\textsc{Output}: Is there a subset repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ such that $w(\aGraph') \geq K$?
\end{minipage}}

\end{center}

\begin{observation}\label{observation:equivalence}
There is a polynomial time algorithm for $\weight$-preferred $\subseteq$-repair computing iff there is a polynomial time algorithm for $K$ $\weight$-preferred repair computing.
\end{observation}

\begin{proof}
The $\implies$ direction is trivial. For the other direction, we can find the optimal value of the repairs $M$ by using binary search on the repair's value (note that this binary search can be done in polynomial time thanks to the conditions we imposed on $\weight$). After that, we can find those edges and nodes that belong to the target repair by removing them and asking to the decision problem solver if there still exists a $M$ valued subset repair. This algorithm runs in polynomial time and does a polynomial number of queries to the decision problem solver. 
\end{proof}

This decision problem is clearly in the class \textsc{NP}, and it is more general than the $\exists$-\textsc{SUBSET-REPAIR} one, which implies that $K$ $\weight$-preferred $\subseteq$-repair computing is \textsc{NP-complete} when $\mathcal{L}$ is \Gregxpath or path expressions from $\Gposregxpath$. When considering only node expressions from $\Gposregxpath$ we noted that the repair is unique, and this means that the decision problem is tractable in that case.

\begin{theorem}
The problem $K$ $\weight-$preferred $\subseteq$-repair computing is \textsc{NP-complete} when $\mathcal{L}$ is \Gregxpath or path expressions from $\Gposregxpath$. It can be solved in polynomial time when $\mathcal{L}$ contains only node expressions from $\Gposregxpath$.
\end{theorem}

\subsubsection{\weight-preferred superset repairs}

Consider the analog problem we defined for subset repairs, but in the context of superset repairs:

\begin{center}

\fbox{\begin{minipage}{30em}
  \textsc{Problem}: \textbf{$K$ \weight-preferred} $\supseteq$-repair computing

\textsc{Input}: A data-graph $\aGraph$, a value $K$ and a set $\aRestrictionSet$ of $\mathcal{L}$ expressions.

\textsc{Output}: Is there a superset repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ such that $w(\aGraph') \leq K$?
\end{minipage}}

\end{center}

Although it is not clear whether we can make an observation similar to Observation~\ref{observation:equivalence} for this problem, it is easy to see that if an algorithm for finding an optimum $\weight$ superset repair exists, then we can solve the previous decision problem, and therefore we can find a lower bound for our repair computing problem using the decision one. 

When using the full power of \Gregxpath we obtain the following result: 

\begin{theorem}
When $\mathcal{L}=\Gregxpath$ there is a set of expressions $\aRestrictionSet$ such that the problem $K$ $\weight$-preferred $\supseteq$-repair computing is \textsc{NP-hard}.
\end{theorem}

\begin{proof}
Observe that if we assign proper values to the edge labels and data values from the proof of Theorem~\ref{teo:NP-hard-data} we can force every superset repair to only add the $\esLabel{value}$ edges to the variable nodes. This means that we can polynomially reduce 3-\textsc{SAT} to $K$ $\weight$-preferred $\supseteq$-repair computing when $\aRestrictionSet$ is fixed.
\end{proof}

For the case of $\Gposregxpath$, note that the polynomial size repair that existed thanks to Theorem~\ref{teo:superset} did not add neither edges or nodes. That is, if there exists a \weight-preferred repair of $\aGraph$ with respect to $\aRestrictionSet$ then it has polynomial size with respect to $|\aGraph|$ and $|\aRestrictionSet|$ (when considering only $\Gposregxpath$ expressions). 

This implies that the decision problem we define is in \textsc{NP} in this case (we can ask for the repair itself as a witness). Now we show that the problem is also \textsc{NP-hard}.

\begin{theorem}\label{teo:Kpreferredsuperset}

There is a set of $\Gposregxpath$ node expressions $\aRestrictionSet$ such that  $K$ \weight-preferred superset repair computing is \textsc{NP-hard}.

\end{theorem}

\begin{proof}

We reduce 3\textsc{-SAT} to the problem $K$ $\weight$-\textbf{preferred} $\supseteq$-repair computing with $\aRestrictionSet$ fixed. For the reduction, we consider $\Sigma_e = \{\esLabel{value\_of}, \esLabel{appears\_in}, \esLabel{appears\_negated\_in}\}$ and $\Sigma_n = \{clause, var, \top,\bot\}$, with the same semantics as in the Theorem~\ref{subsetRepairNPcomplete}\sergio{Broken reference}. We define the weight function $w$ as $w(c) = 2$ for $c \in \Sigma_n \cup \{\esLabel{appears\_in}, \esLabel{appears\_negated\_in}\}$ and $w(\esLabel{value\_of)} = 1$.

Given a 3\textsc{-CNF} formula $\phi$ with $n$ variables and $m$ clauses we build a data-graph $\aGraph$, a set of $\Gposregxpath$ node expressions $\aRestrictionSet$ and define a number $K$ such that $\phi$ is satisfiable if and only if $\aGraph$ has a superset repair $\aGraph'$ with respect to $\aRestrictionSet$ such that $w(\aGraph') \leq K$.

The graph is similar to the one used in Theorem~\ref{subsetRepairNPcomplete}, and we define it as $G=(V_\aGraph, L_\aGraph, D_\aGraph)$ where:

\begin{center}
    
    $V_\aGraph = \{x_i$ $|$ $1 \leq i \leq n\}$ $\cup$ $\{c_j$ $|$ $1\leq j \leq m\}$ $\cup$ $\{\bot, \top\}$
    
    \bigskip 
    
    $L_\aGraph(x_i,c_j) =$  $\begin{cases} 
      \{\esLabel{appears\_in}, \esLabel{appears\_negated\_in}\}\text{ if } x_i \text{ and } \lnot x_i \text{ appear in }c_j \\
      \{\esLabel{appears\_in}\}\text{ if } x_i \text{ appears in }c_j \\
      \{\esLabel{appears\_negated\_in}\}\text{ if }\lnot x_i \text{ appears in }c_j \\
      \emptyset \text{ otherwise} 
   \end{cases}$
   
   $L_\aGraph(v,w) = \emptyset$ for every other pair $v,w \in V_\aGraph$
   
   \bigskip
   
   $D(\bot) = \bot$, $D(\top) = \top$
   
   $D(x_i) = var$ for $1\leq i \leq n$
   
   $D(c_j) = clause$ for $1 \leq j \leq m$

    
\end{center}

The structure of $\phi$ is codified in the \esLabel{appear} edges. We define $K=w(\aGraph) + n$, and we want any superset repair of $\aGraph$ with respect to $\aRestrictionSet$ with weight $K$ to codify an assignment of the `node' variables by using the edges \esLabel{value\_of}. In order to do this we define the \Gposregxpath expressions

\begin{equation}\label{teo:allValueEdges}
    \aFormulab_1 = \comparacionCaminos{[var^{\neq}] \cup \down_\esLabel{value\_of} [\top] \cup \down_\esLabel{value\_of} [\bot]}
\end{equation}

\begin{equation}\label{teo:allSatisClauses}
    \aFormulab_2 = \comparacionCaminos{ [clause^{\neq}] \cup \down_\esLabel{appears\_in}^- \down_\esLabel{value\_of} [\top] \cup \down_\esLabel{appears\_negated\_in}^- \down_\esLabel{value\_of} [\bot]}
\end{equation}

The expression~\ref{teo:allValueEdges} forces every Variable node to have a \esLabel{value} edge directed to a Boolean node, while the expression~\ref{teo:allSatisClauses} forces every clause to be `satisfied' in any repair of $\aGraph$. Therefore, we define $\aRestrictionSet = \{ \aFormulab_1, \aFormulab_2\}$. Now we show that $\phi$ is satisfiable if and only if $\aGraph$ has a superset repair with respect to $\aRestrictionSet$ with weight at most $w(\aGraph) + n$.

$\implies)$ Let $f$ be a valuation on the variables of $\phi$ that evaluates $\phi$ to true. We then `add' edges to $\aGraph$ in the following way: if $f(x_i) = \top$ we add the edge $(x_i,\esLabel{value\_of},\top)$, and otherwise we add $(x_i,\esLabel{value\_of},\bot)$. This graph satisfies both expressions from $\aRestrictionSet$ and has cost $w(\aGraph) + n$, since $w(\esLabel{value\_of}) = 1$.

$\impliedby)$ Let $\aGraph'$ be a superset repair of $\aGraph$ with respect to $\aRestrictionSet$ with weight at most $w(\aGraph) + n$. Since every superset repair of $\aGraph$ has to add at least $n$ \esLabel{value} edges, and they cost 1 unit each, we know that $\aGraph'$ has to be exactly the original graph $\aGraph$ plus $n$ \esLabel{value} edges (one for each node variable). Then we can define a valuation of the variables of $\phi$ by using this edges: if the edge $(x_i,\esLabel{value\_of}, \top)$ is present in $\aGraph'$ we define $f(x_i) = \top$, and otherwise $f(x_i) = \bot$. Since $\aFormulab_2$ is satisfied in $\aGraph'$ this assignment must satisfy $\phi$.

\end{proof}

Therefore, we can conclude that

\begin{corollary}
The problem $K$ $\weight$-preferred superset repair is \textsc{NP-complete} when $\mathcal{L}=$\Gposregxpath.
\end{corollary}

\subsection{Multiset-based preferences}
%\subsection{Lifting an order over edges and data to multiset orderings}
\bigsergio{Contar acá que vamos a trabajar en quasi-orders (hablar de la utilidad de eso), pero que para eso empezamos por partial orders }
Given a set $A$, its set of finite multisets $\multiset{A}$ is formally defined as $$\multiset{A} =\{f:A \to \N \mid  \mbox{{\small $\{x \mid f(x) \neq 0\}$} is finite}\}.$$ 

For two multisets $M_1, M_2$, we usually use the notation $M_1\cup M_2$ to indicate the multiset $M_1 + M_2$, and represent multisets as if they were sets with repetition (e.g. $\{0,3, 3, 4,4,4,10\}$).

%We say that $x \in \multiset{A}$ if $f(x) > 0$.
Given a strict partial order $(A, <)$, the multiset ordering over $\multiset{A}$ (i.e. the multiset extension $(\multiset{A}, \lessMultiset)$) is defined as follows (taken from \cite{DershowitzManna, huet1980equations}). %$M_1 \lessMultiset M_2$ iff $M_1 = (M_2 \backslah X) \cup Y$ for some $A,B \in \multiset{A}$, with $\emptyset \neq X \subseteq M_2$, and for 
%When $(A, \le)$ is a partial order,
$M_1 \lessMultiset M_2$ iff $M_1 \neq M_2$ and for all $x \in A$, if $M_1(x) > M_2(x)$, then there exists some $y \in A$ such that $x < y$ %, $x \le y$, x \not \ge y$, 
and  $M_1(y) < M_2(y)$.
When $(A, <)$ is a total order, the definition is equivalent to: 
$M_1 \lessMultiset M_2$ iff $M_1 \neq M_2$ and, if $d = \max\{z \in A \mid M_1(z) \neq M_2(z)\}$, we have that $M_1(d) < M_2(d)$.

\begin{example} Over $\multiset{\N}$ we have $\{0,0,0,1,1,1,2\} \lessMultiset \{2,2\}$. \end{example}

If $(A, <)$ is a strict partial (resp. total) order, then $(\multiset{A}, \lessMultiset)$ is a partial (resp. total) order. If $(A, <)$ is a well-founded order\footnote{I.e. for all $S \subseteq A$, if $S \neq \emptyset$ then there exists $m \in S$ such that there is no $s \in S$ such that $s<m$.}, so is $(\multiset{A}, \lessMultiset)$\cite{DershowitzManna}. 




%\paragraph{Lifting a partial order over edges and data values to preferences over multisets}
\paragraph{Lifting a partial order to preferences via  multisets}\label{subsection:PartialOrderPreferenceMultisets}
% La versión anterior, solo sobre edges, la dejé archivada en oldMultisetEdges.tex
We first consider the case where there is a partial ordering over edges and data values, which we aim to lift to some multisets which induce a notion of preference over the underlying data-graphs. 

\begin{definition}
Given a data-graph $G = (V,L_e,D)$, we define its \defstyle{multiset of edges and data values} as the multiset: 
$$\edgeDataMultiset{G} = \bigcup_{x,y \in V} L_e(x,y) \cup \bigcup_{x \in V} D(x) $$
\end{definition}

\begin{definition}\label{definition:MultisetPreferencesFromPartialOrder}
Let $G_1, G_2$ be two data-graphs over $\Sigma_e$ and $\Sigma_n$, and let $<$ be a partial order defined over the (disjoint) union $\Sigma_e \sqcup \Sigma_n$. 
We say that $G_1 \lessPreferedInducedMultiset G_2$ ($G_1$ is \defstyle{multiset-preferred} to $G_2$) if: 
$$\edgeDataMultiset{G_1} \lessMultiset \edgeDataMultiset{G_2} $$

We say that $G_1 \equivalentPreferedInducedMultiset G_2$ if:  
$$\edgeDataMultiset{G_1} = \edgeDataMultiset{G_2} $$
\end{definition}

\begin{observation}
The relation $\lessEquivalentPreferedInducedMultiset = \lessPreferedInducedMultiset \cup \equivalentPreferedInducedMultiset$ over data-graphs (over fixed $\Sigma_e, \Sigma_n$) is a quasi-ordering (i.e. reflexive and transitive). 
\end{observation}

\begin{observation}
If $<$ is a well-founded order, then any set of data-graphs has at least one $\lessPreferedInducedMultiset$-minimum, but many of these graphs could map to that same multiset.
If the set of nodes is fixed and finite, the size of each equivalence class of $\equivalentPreferedInducedMultiset$ is finite.
\end{observation}

\begin{remark}
When using multiset preferences for superset repairs, edges/values with a lower `position' on $(\Sigma, <)$ will be preferentially added. In a subset repair, edges/values with a high position will be preferentially removed. 
\end{remark}

\begin{example} Consider a database that represents road accessibility between geographical points. When two points are linked via a road, it must be also indicated whether the connection is via an asphalt road or a dirt road. Consider an ordering over the set of labels such that $\esLabel{dirt} < \esLabel{asphalt} < \esLabel{road}$, and a set of restrictions $\aRestrictionSet = \{\alpha_{road-type-specified}\}$,
%\sergio{En realidad también tendría sentido pedir que resulte un grafo planar, pero no sé si se puede hacer con esta lógica}%by Shay Mozes, "Truly subquadratic exact distance oracles with constant query time for planar graph"https://zoom.us/rec/share/1-1cIBoyGe440F-LXyrs6hQVsVwdvHUIU4WymhmtI_THALqKMIM3maOI-nijTe2G.aKx5Zkq2eKYF9k7Q?startTime=1614602531000
 which forces connected points to more precisely distinguish the type of road that connects them: $$\alpha_{road-type-specified} = \esLabel{road} \entoncesCamino \esLabel{dirt} \unionCaminos \esLabel{asphalt}.$$ 

In these conditions, a superset repair based on multiset preferences represents a conservative assumption that a road between two places is of low quality rather than high.
Note that in the same conditions, a subset repair will preferentially remove altogether the \esLabel{road} connection between the points.
\end{example}


\begin{example}\label{example:BadBehaviourPartialOrderMultisetPreferences} 
Let $\Sigma_e = \{\downarrow\}$, $\Sigma_n = \{\aData, \aDatab, \esDato{r}\}$. $G$ consists of a single node with data value $\aData$. Let 
$\aRestrictionSet = \{\varphi, \aPath_{noCycles}\}$, where we have $\aPath_{noCycles} = \epsilon \entoncesCamino \overline{\_^+}$ and where $\varphi = \esDatoIgual{\aData} \entoncesNodo (\comparacionCaminos{\downarrow \expNodoEnCamino{\esDatoIgual{\esDato{r}}}} \lor \comparacionCaminos{(\downarrow\expNodoEnCamino{\esDatoIgual{\aDatab}})^{1000,1000}})$.
If our order over $\Sigma_e \sqcup \Sigma_n$ is given by $\downarrow < \aData < \aDatab < \esDato{r}$, a superset repair adding a thousand new nodes (with data values $\aDatab$) and edges $\downarrow$ (see Figure~\ref{figure:multisetExampleMultisetPreferredRepair}) will be preferred to a simpler one where we only need to add one node with value $\esDato{r}$ and one edge (see Figure~\ref{figure:multisetExampleRepair}).

\begin{figure} [H]
\centering
    \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
\node[main] (1) {\aData}; 
\node[main] (2) [right of=1] {\esDato{r}}; 
\draw[->] (1) edge node[midway, below=0.5pt, sloped, pos=0.5]{} (2);
%\draw[->, bend left = 30] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{high} (4); 
%\draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\end{tikzpicture} 
\caption{A superset repair for the singleton datagraph $\aGraph$ from Example~\ref{example:BadBehaviourPartialOrderMultisetPreferences}}
\label{figure:multisetExampleRepair}
\end{figure}


\begin{figure} [H]
\centering
    \begin{tikzpicture}[node distance={45mm}, thick, main/.style = {draw, rectangle}] 
\node[main] (1) {\aData}; 
\node[main] (2) [right of=1] {\aDatab}; 
\node[main] (3) [right of=2] {\aDatab}; 
\node[main] (4) [right of=3] {\aDatab}; 
\draw[->] (1) edge node[midway, below=0.5pt, sloped, pos=0.5]{} (2);
\draw[->] (2) edge[dotted] node[midway, below=2.5pt, sloped, pos=0.5]{998 instances of $\downarrow$ and a node with $\aDatab$} (3);
\draw[->] (3) edge node[midway, below=0.5pt, sloped, pos=0.5]{} (4);
%\draw[->, bend left = 30] (1) edge node[midway, above=0.5pt, sloped, pos=0.5]{high} (4); 
%\draw[->] (1) -- (2) node[midway, above=0.5pt, sloped, pos=0.5]{low};
\end{tikzpicture} 
\caption{A multiset-preferred superset repair for $\aGraph$ from Example~\ref{example:BadBehaviourPartialOrderMultisetPreferences}, given the underlying order  $\downarrow < \aData < \aDatab < \esDato{r}$.}
\label{figure:multisetExampleMultisetPreferredRepair}
\end{figure}


\end{example}



Requiring a partial ordering over $\Sigma_e \sqcup \Sigma_n$ can be too restrictive when constructing preferences based on the resulting multisets. For example, if the data value $\aData$ is smaller than $\aDatab$ ($\aData < \aDatab$), then a superset repair that only needs the single addition of a node with $\aData$ could be less preferred to a repair requiring an arbitrarily high number of added $\aDatab$ values (depending on what other elements are added besides these nodes). See Example~\ref{example:BadBehaviourPartialOrderMultisetPreferences} for a toy model of this kind of situation.
This behavior might be unwarranted when there is small semantic distance between the data values, such as between $\esDato{3000}$ and $\esDato{3001}$ in a database where data values represent prices in dollars, or when we want groupings between types of data values but without imposing an order within each group, such as when data values can be either proper names from authors or titles from books.
These types of behavior can be avoided or improved by relaxing the requirements of the underlying relation over $\Sigma_e \sqcup \Sigma_n$, and merely asking for it to be a quasi-order: a reflexive and transitive relation. This definition allows for many elements to belong to the same equivalence class derived from $\le$, which is a way to group  elements that are semantically similar or equally preferred.

We specify this broader definition as follows.


%\paragraph{Lifting a quasi-order over edges and data values to preferences over multisets}
\paragraph{Lifting a quasi-order to preferences via multisets}
If $\Sigma = \Sigma_e \sqcup \Sigma_n$ has merely an associated quasi-ordering $\le_q$ (i.e. a reflexive and transitive relation), we take the quotient set of equivalence classes of the equivalence relation given by the definition $x \equiv y \Leftrightarrow x \le_q y \land y \le_q x$, thus obtaining a partial ordering $({\Sigma}_{\slash \equiv}, \le)$ from which we can extract a strict partial ordering $({\Sigma}_{\slash \equiv}, <)$. 
Thus, by applying this quotient, we can extend our definition of multiset-preferred data-graphs  % of Section~\ref{subsection:PartialOrderPreferenceMultisets} 
from partial orders to the case where the underlying relation on $\Sigma$ is a quasi-order. 

\begin{definition}\label{definition:MultisetPreferencesFromQuasiOrder}
Let $G_1, G_2$ be two data-graphs over $\Sigma_e$ and $\Sigma_n$, and let $\le_q$ be a partial order defined over the disjoint union $\Sigma_e \sqcup \Sigma_n$. 
%If $G_1, G_2$ are data graphs over $\Sigma_e$ and $\Sigma_n$, such that $(\Sigma_e \sqcup \Sigma_n, \le_q)$ is a quasi-order, we define: 
From $(\Sigma, \le_q)$ we define $({\Sigma}_{\slash \equiv}, <)$ as was done above. 
Our notion of \emphstyle{multiset-preferred} is given by: 
$$G_1 \lessPreferedInducedMultiset G_2 \text{ iff } \edgeDataMultiset{{G_1}}_{\slash \equiv} \lessMultiset^{({\Sigma}_{\slash \equiv}, <)} \edgeDataMultiset{{G_2}}_{\slash \equiv},$$
where for all $[x] \in {\Sigma}_{\slash \equiv}$ we have:
$$\edgeDataMultiset{{G_i}}_{\slash \equiv}([x]) = \sum_{y \in [x]} \edgeDataMultiset{G_i}(y) $$

We also define:  $$G_1 \equivalentPreferedInducedMultiset G_2 \text{ iff }
\edgeDataMultiset{{G_1}}_{\slash \equiv} = \edgeDataMultiset{{G_2}}_{\slash \equiv} $$
\end{definition}

%In other words, when $\Sigma$ is a quasi-order, edges and data values could be counted as having the same `priority' (none are preferred over the other), or they could have some strict preference between them, or instead they could be mutually incomparable. 

\begin{observation}
Definition~\ref{definition:MultisetPreferencesFromQuasiOrder} is effectively an extension of Definition~\ref{definition:MultisetPreferencesFromPartialOrder}, since they coincide when the underlying order is a partial order (the equivalence classes over a partial order are singletons).
\end{observation}




\begin{remark}
While in full generality we can consider any ordering over $\Sigma_e \sqcup \Sigma_n$, in many domains it will make more sense to consider that $\Sigma_e$ and $\Sigma_n$ have their own orderings, and then we consider the disjoint ordering over their union. 
\end{remark}


\begin{remark}
Depending on the domain of use of a database, it could happen that nodes have a particular relevance or trustworthiness, and thus we do not want to add or remove them except as a last resort, preferring instead to exhaust all possibilities with edges first. 
This can be easily done via multiset preferences via a correct selection of the underlying ordering. 

Suppose that we are using superset repairs. Then, we want an ordering such that all data values are equivalent and such that any data value is larger than any edge-label, that is: from $(\Sigma_e, <)$ we construct the quasi-order $(\Sigma_e \sqcup \Sigma_n, \le')$, via $x \le' y$ iff $x=y$, or $x,y\in \Sigma_e$ and $x<y$, or $x,y \in \Sigma_n$, or $x \in \Sigma_e, y\in \Sigma_n$. Here, all nodes have the same priority, but all nodes have a higher priority than all edges. 

Note that in the case of subset repairs, we should instead switch the priorities so that edges dominate data values, and thus edge-labels are removed preferentially. 
\end{remark}



\begin{example} Let $(\Sigma, \le)$ be some quasi-order and let $\top$ be a fresh edge label (such that $\top \not \in \Sigma$). We consider $\Sigma_{+} = \Sigma +\{\top\} = (\Sigma \sqcup \{\top\}, \le_{+\top} )$ as the extension of $\Sigma$ so that $\forall x, x \le_{+\top} \top$. Observe that if $\Sigma$ was a total well-ordering, then so is $\Sigma_{+}$.

When considering a preference over subset repairs, orders like that of $\Sigma_{+}$ can be useful to always prioritize the removal of edges with a particular sensitive label over the removal of others. Consider, for example, a label that represents having administrator privileges or a high security clearance. 
\end{example}

\paragraph{Computing multiset-preferred repairs}

We define the following problem:

\begin{center}

\fbox{\begin{minipage}{30em}
  \textsc{Problem}: \textbf{multiset-preferred} $\star$-repair computing

\textsc{Input}: A data-graph $\aGraph$ and a set $\aRestrictionSet$ of $\mathcal{L}$ expressions.

\textsc{Output}: A $\star$-repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ such that there is no other repair $H$ that is \textbf{multiset-preferred} to $G'$.
\end{minipage}}

\end{center}

where $\star \in \{\subseteq, \supseteq\}$. We assume a  fixed strict partial ordering $(\Sigma, <)$ over the set $\Sigma = \Sigma_e \sqcup \Sigma_n$ of data values and edge labels. As we did in the $\weight$-preferred repair section, we condition the strict partial order to be efficiently computable: we assume that given two elements $x,y \in \Sigma_e \sqcup \Sigma_n$ we can decide if $x<y$ in polynomial time with respect to the codification size of $x$ and $y$.

To study the repair computing problem under this preference semantics, we define the following decision problem:

\begin{center}

\fbox{\begin{minipage}{30em}
  \textsc{Problem}: \textbf{multiset-preferred} $\star$-repair bound

\textsc{Input}: A data-graph $\aGraph$, a set $\aRestrictionSet$ of $\mathcal{L}$ expressions and an element $d \in \Sigma_n \sqcup \Sigma_e$.

\textsc{Output}: Is there a multiset preferred $\star$-repair of $\aGraph$ with respect to $\aRestrictionSet$ such that there is no element $d' \in \Sigma_n^\aGraph \sqcup \Sigma_e^\aGraph$ that satisfies $d<d'$?
\end{minipage}}

\end{center}

This decision problem is similar to the one defined for the $\weight$-preferred semantics: we want to decide if $d$ is a kind of `upper bound' (based on the order $<$) on the elements of a multiset preferred repair of $\aGraph$ with respect to $\aRestrictionSet$.

\subsubsection{Multiset-preferred subset repairs}

In the case of subset repairs, it is clear that the problem is in \textsc{NP}, since for a positive certificate it is enough to show a data-graph $\aGraph'$ and check that $\aGraph' \subseteq \aGraph$, $\aGraph' \models \aRestrictionSet$ and that for every $d' \in \Sigma_n^{\aGraph'} \sqcup \Sigma_e^{\aGraph'}$ it happens that $d \nless d'$.

If $\mathcal{L}$ only contains node expressions from $\Gposregxpath$ the problem is trivial, since we know that there is a unique subset repair and that we can compute it in polynomial time due to Theorem~\ref{teo:uniqueSubsetRepair}. Meanwhile, if $\mathcal{L} = \Gposregxpath$, the problem is \textsc{NP-hard}.

\begin{theorem}
The problem multiset-preferred $\subseteq$-repair bound is $\textsc{NP-hard}$ when $\mathcal{L}=\Gposregxpath$, even when $\aRestrictionSet$ is fixed.
\end{theorem}

\begin{proof}

We can use the same reduction from the proof of Theorem~\ref{teo:subsetPositiveIntractable}, adding a new data value $c$ to the set-up which will be used as the $d$ bound from our problem, and defining an order $<$ such that $c \nless d'$ for every other element $d'$.

\end{proof}

\subsubsection{Multiset-preferred superset repairs}

As we have already seen, finding a superset repair is an intractable problem (even when $\aRestrictionSet$ is fixed) when allowing the full power of \Gregxpath for the restriction set, and therefore we only consider the case when every expression belongs to the \Gposregxpath fragment.

We note, once again, that the conversion in Theorem~\ref{teo:superset} does not add neither edges nor data values. Then we know that if there exists a multiset preferred superset repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ bounded by $d$ then there has to be one with the `standard' form: one that adds to $\aGraph$ one node for each new data value in $\Sigma_n^{\aGraph'} \setminus \Sigma_n^{\aGraph}$. This implies that if the answer to the decision problem is positive we can find a certificate of polynomial size on $|\aGraph| + |\aRestrictionSet|$, and we can conclude that the problem is in \textsc{NP}.

As we have seen when studying the $\exists$\textsc{SUPERSET-REPAIR} problem, letting $\aRestrictionSet$ be a parameter and $\Sigma_n$ be infinite made the problem difficult. In this case, the same holds:

\begin{theorem}
If $\aRestrictionSet$ is unfixed and $\Sigma_n$ can be infinite, there is a set-up where the problem multiset preferred $\supseteq$-repair bound is \textsc{NP-hard}.
\end{theorem}

\begin{proof}
We can use the reduction from the proof of Theorem~\ref{teo:supsetHardInfinite} in a similar way as we did previously: we define a new data value $c$ to the set-up that will be used as $d$ and an order $<$ such that $c \nless d'$ for every element $d'$. Then asking for the existence of a superset repair in that context reduces to ask for the existence of a superset repair where $c$ works as a bound (i.e. $c \nless d'$ for every $d'$ in the repair).
\end{proof}

Meanwhile, if $\aRestrictionSet$ is fixed or $\Sigma_n < \infty$ the problem is tractable, since we can use a procedure similar to algorithm 2:

\begin{algorithm}[H]
\begin{algorithmic}[1]
\REQUIRE $\aGraph$ is a datagraph, $\aRestrictionSet$ a set of $\Gposregxpath$ expressions and $d \in \Sigma_n \cup \Sigma_e$.
\STATE $c_1,c_2 \leftarrow \text{two data values such that }d \nless c_i\text{ and } c_i \notin \Sigma_n^\aRestrictionSet \cup \Sigma_n^\aGraph \text{ (if possible)}$
\STATE $\Sigma_n^{d \nless}$ $\leftarrow$ \text{edge labels } $e$ \text{ such that }$d \nless e$
\FOR{$S \in \mathcal{P}(\Sigma_n^{\aRestrictionSet_d} \cup \{c_1,c_2\} \setminus \Sigma_n^\aGraph)$}
    \STATE $H \leftarrow buildGraph(\aGraph, S, \Sigma_n^{d \nless})$
    \IF{$H \models \aRestrictionSet$ and is bounded by $d$}
        \RETURN $H$ as a positive certificate
    \ENDIF
\ENDFOR

\RETURN There is no superset repair with $d$ as bound


\end{algorithmic}
\caption{$SupersetRepairBound(\aGraph,\aRestrictionSet,d)$}
\end{algorithm}

%$\aGraph$ is a datagraph, $\aRestrictionSet$ a set of $\Gposregxpath$ expressions and $d \in \Sigma_n \cup \Sigma_e$ 

The function \textit{buildGraph}$(\aGraph,S,\Sigma)$ makes a new graph by adding to $\aGraph$ one node $v_c$ for each data value $c \in S$, defining $D(v_c) = c$ and adding the edge labels from $\Sigma$ between every pair of nodes. Now we show the correctness of the algorithm:

\begin{theorem}
Given a data-graph $\aGraph$, a set of \Gposregxpath expressions $\aRestrictionSet$ and a bound $d$ the algorithm SupersetRepairBound outputs a certificate $H$ if and only if $\aGraph$ has a multiset-preferred superset repair with respect to $\aRestrictionSet$ bounded by d.
\end{theorem}

\begin{proof}
$\implies$) Suppose the algorithm outputs a data-graph $H$. Since $H \models \aRestrictionSet$ there must exist a superset repair $\aGraph'$ of $\aGraph$ with respect to $\aRestrictionSet$ contained in $H$. If $\aGraph'$ is also multiset-preferred we are done, since $\aGraph'$ is bounded by $d$, but otherwise suppose that there is another superset repair $I$ such that $I <_{Gmset} \aGraph'$ and that there is no other repair $I'$ such that $I' <_{Gmset} I$. We show that $I$ is bounded by $d$.

By contradiction, let there be an element $d'$ in $I$ such that $d < d'$. Since $I <_{Gmset} \aGraph'$ we know that either $\aGraph'$ contains a quantity of $d'$ elements bigger or equal than $I$'s, or that there is another element $d''$ such that $d' < d''$ and $G'(d'') > I(d'')$. The first case cannot hold, because in that scenario $\aGraph'$ contains an element bigger than $d$ (according to the order), and by construction $\aGraph'$ only contains elements of $H$, which didn't contain any element bigger than $d$. The second case cannot hold either, since by the transitivity of $<$ we can deduce that $d < d''$, which implies that once again $H$ contained an element bigger than $d$. 

Then there exists a multiset preferred superset repair of $\aGraph$ with respect to $\aRestrictionSet$ bounded by $d$.

$\impliedby$) Let's assume that $\aGraph$ has a multiset-preferred repair $\aGraph'$ with respect to $\aRestrictionSet$ that is bounded by $d$. Observe that $\aGraph'$ has to be in standard form, since otherwise we can contract two nodes with the same data value to build a smaller repair (which will be preferred due to the multiset semantics). Observe that we can also use Lemma~\ref{teo:dataValuesInR} to conclude that given $\aGraph'$ we can construct a new data-graph $K$ that only uses at most two extra data values from those mentioned in $\Sigma_n^R \cup \Sigma_n^\aGraph$ and also satisfies $\aRestrictionSet$. Following the proof of Lemma~\ref{teo:dataValuesInR} we pick two different data values $c_1$ and $c_2$ in $\Sigma_n^{G'} \setminus (\Sigma_n^R \cup \Sigma_n^\aGraph)$ and change the data values of every other node with data value different from $c_1$ and $c_2$ to $c_1$. We can then contract every node with value $c_1$, while still being consistent with $\aRestrictionSet$. Let's call this last graph $K'$.

By construction, every element $x$ from $K'$ satisfies $d \nless x$ (note that we began with $\aGraph'$ which was bounded by $d$, and we obtained $K'$ by deleting elements from $\aGraph'$ or adding data values already in $\aGraph'$) and $K'$ is in standard form. Also, the set of edges that $K'$ uses is clearly a subset of $\Sigma_n^{d\nless}$. Observe that if we `complete' $K'$ by adding between every node the edges $\Sigma_n^{d\nless}$ then the resulting data-graph $K''$ still satisfies $\aRestrictionSet$ due to \ref{monotony}, and it is also bounded by $d$. 

Suppose that $K''$ has two extra data values $f_1$ and $f_2$ from those mentioned in $\aRestrictionSet$, and let $c_1$ and $c_2$ be the data values chosen by the algorithm in the first step. It is clear that if we change the data value $f_1$ and $f_2$ in $K''$ for $c_1$ and $c_2$ the resulting data-graph will satisfy $\aRestrictionSet$, since none of these values is mentioned in $\aRestrictionSet$, and every data inequality that interacts with the data values $c_1$ and $c_2$ will still be satisfied. Then observe that this data-graph $K''$ will be found by the algorithm, and it will output the certificate $H=K''$



\end{proof}

\begin{corollary} If the first line of algorithm 3 can be computed in polynomial time in the input size, then the problem multiset-preferred $\supseteq$-repair bound problem can be solved in polynomial time when $\mathcal{L} = \Gposregxpath$ and either $\Sigma_n$ is finite or $\aRestrictionSet$ is fixed
\end{corollary}

This follows by assuming that the first line of the algorithm can be computed efficiently and observing that the number of iterations is bounded by a constant if either $\aRestrictionSet$ is fixed or $\Sigma_n$ is finite.

The assumption that the first line can be computed is reasonable if the order is such that, given an element $d$, it is possible to enumerate efficiently the set of elements X such that $d \nless x$ for all $x \in X$. This would happen, for example, if the order $<$ represents lexicographical ordering.

